SFlexRCA: Lightweight, Scalable, and Flexible Root Cause Analysis for IIoT Edge Systems

Industrial Internet of Things (IIoT) systems generate high-dimensional sensor telemetry from interconnected components, where faults can propagate across the system. To address these challenges, we propose SFlexRCA (Scalable and Flexible Root Cause Analysis), a topology-free RCA framework designed for resource-constrained IIoT environments. SFlexRCA transforms multivariate telemetry into compact orthogonal representations and applies shared lightweight linear modeling, avoiding explicit graph construction, message passing, and per-variable or lag-specific parameter growth. We evaluate SFlexRCA on three publicly available IIoT datasets, BATADAL, SWaT, and WADI, spanning different numbers of monitored variables, temporal characteristics, and training-data regimes. SFlexRCA is compared with 10 statistical, causal, and non-causal baselines in terms of RCA accuracy, training efficiency, inference latency, and memory consumption. In addition, inference efficiency and memory consumption are evaluated on Raspberry Pi 3 and Raspberry Pi 5, while energy consumption is additionally measured on Raspberry Pi 5. We further investigate temporalcontext sensitivity, architectural and loss components, and alternative representations. Notably, SFlexRCA maintains strong localization performance on BATADAL despite its limited normal-operation training data, while its compact shared architecture avoids the parameter growth associated with causal and graph-based approaches. Its lightweight shared architecture further enables efficient deployment on resource-constrained IIoT edge devices. The SFlexRCA code is available at https://github.com/theamrzaki/RootCause- Analysis-Correlation-Attentive-Modeling.

==> sections/DataAval.tex <==
\section*{Data Availability}

In accordance with the open science policy of ESEM 2026, we provide access to the artifacts required to reproduce the main experimental results of this study.

The source code, experimental scripts, and model configurations are available via a private Figshare repository:
\textit{https://figshare.com/s/a365f4b6c82098858644?file=64699461}.

The repository includes evaluation scripts, training pipelines, hyperparameters and configurations used for all reported experiments, including ablation studies and figure generation. Additional evaluation metrics (e.g., MRR, and Hit Rate) as well as full training logs are also provided to support extended analysis beyond the results reported in the paper due to space constraints.

All datasets used in this study are based on publicly available benchmarks (SMD, AIOps, and GAIA) and do not contain sensitive or proprietary information. Preprocessing procedures, evaluation protocols, and hyperparameter settings are fully documented in the repository to ensure reproducibility.

==> sections/exps/__wadi_swat_projections.tex <==


\begin{figure*}[t]
    \centering
    % Row 1: Baselines & First 2 Static Projections
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_swat_ws_8_seed_1_numvars_51_transformation_none_none_tsne.pdf}
        \caption{None (Baseline)}
        \label{fig:tsne_swat_none}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_swat_ws_8_seed_1_numvars_51_transformation_learned_learned_tsne_2.pdf}
        \caption{Learned}
        \label{fig:tsne_swat_learned}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_swat_ws_8_seed_1_numvars_51_transformation_legendre_legendre_tsne_2.pdf}
        \caption{Legendre}
        \label{fig:tsne_swat_legendre}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_swat_ws_8_seed_1_numvars_51_transformation_laguerre_laguerre_tsne_2.pdf}
        \caption{Laguerre}
        \label{fig:tsne_swat_laguerre}
    \end{subfigure}
    
    \vspace{0.8em} % Spacing between rows
    
    % Row 2: Remaining Static Projections & Proposed Method
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_swat_ws_8_seed_1_numvars_51_transformation_chebyshev_chebyshev_tsne_2.pdf}
        \caption{Chebyshev}
        \label{fig:tsne_swat_chebyshev}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_swat_ws_8_seed_1_numvars_51_transformation_hermite_hermite_tsne_2.pdf}
        \caption{Hermite}
        \label{fig:tsne_swat_hermite}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_swat_ws_8_seed_1_numvars_51_transformation_fourier_fourier_tsne_2.pdf}
        \caption{Fourier}
        \label{fig:tsne_swat_fourier}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_swat_ws_8_seed_1_numvars_51_transformation_orthogonal_orthogonal_tsne.pdf}
        \caption{Orthogonal (Proposed)}
        \label{fig:tsne_swat_orthogonal}
    \end{subfigure}
    
    \caption{t-SNE latent feature projections on the SWaT dataset corresponding to baseline methods, static polynomial/frequency projections, and our proposed orthogonal projection (matching Table~\ref{tab:RQ5}).}
    \label{fig:tsne_grid_swat}
\end{figure*}



\begin{figure*}[t]
    \centering
    % Row 1: Baselines & First 2 Static Projections
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_wadi_ws_8_seed_1_numvars_127_transformation_none_none_tsne.pdf}
        \caption{None (Baseline)}
        \label{fig:tsne_wadi_none}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_wadi_ws_8_seed_1_numvars_127_transformation_learned_learned_tsne_2.pdf}
        \caption{Learned}
        \label{fig:tsne_wadi_learned}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_wadi_ws_8_seed_1_numvars_127_transformation_legendre_legendre_tsne_2.pdf}
        \caption{Legendre}
        \label{fig:tsne_wadi_legendre}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_wadi_ws_8_seed_1_numvars_127_transformation_laguerre_laguerre_tsne_2.pdf}
        \caption{Laguerre}
        \label{fig:tsne_wadi_laguerre}
    \end{subfigure}
    
    \vspace{0.8em} % Spacing between rows
    
    % Row 2: Remaining Static Projections & Proposed Method
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_wadi_ws_8_seed_1_numvars_127_transformation_chebyshev_chebyshev_tsne_2.pdf}
        \caption{Chebyshev}
        \label{fig:tsne_wadi_chebyshev}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_wadi_ws_8_seed_1_numvars_127_transformation_hermite_hermite_tsne_2.pdf}
        \caption{Hermite}
        \label{fig:tsne_wadi_hermite}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_wadi_ws_8_seed_1_numvars_127_transformation_fourier_fourier_tsne_2.pdf}
        \caption{Fourier}
        \label{fig:tsne_wadi_fourier}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/RQ5/zip/vlinear_wadi_ws_8_seed_1_numvars_127_transformation_orthogonal_orthogonal_tsne_2.pdf}
        \caption{Orthogonal (Proposed)}
        \label{fig:tsne_wadi_orthogonal}
    \end{subfigure}
    
    \caption{t-SNE latent feature projections on the WADI dataset corresponding to baseline methods, static polynomial/frequency projections, and our proposed orthogonal projection (matching Table~\ref{tab:RQ5}).}
    \label{fig:tsne_grid_wadi}
\end{figure*}

